DICT-MLM: Improved Multilingual Pre-Training using Bilingual Dictionaries

Pre-trained multilingual language models such as mBERT have shown immense gains for several natural language processing (NLP) tasks, especially in the zero-shot cross-lingual setting. Most, if not all, of these pre-trained models rely on the masked-language modeling (MLM) objective as the key language learning objective. The principle behind these approaches is that predicting the masked words with the help of the surrounding text helps learn potent contextualized representations. Despite the strong representation learning capability enabled by MLM, we demonstrate an inherent limitation of MLM for multilingual representation learning. In particular, by requiring the model to predict the language-specific token, the MLM objective disincentivizes learning a language-agnostic representation -- which is a key goal of multilingual pre-training. Therefore to encourage better cross-lingual representation learning we propose the DICT-MLM method. DICT-MLM works by incentivizing the model to be able to predict not just the original masked word, but potentially any of its cross-lingual synonyms as well. Our empirical analysis on multiple downstream tasks spanning 30+ languages, demonstrates the efficacy of the proposed approach and its ability to learn better multilingual representations.

==> background.tex <==
\section{Background}
Masked language modeling (MLM), also referred as the \textit{Cloze} test \cite{taylor1953cloze}, was first proposed by \citet{devlin-etal-2019-bert} to train deep bi-directional contextualized representations. Given an input text stream $W\!=\!w_1, w_2 \cdots w_n$,  MLM uses the past and future tokens $W_{\setminus t}\!:=\!(w_1,\cdots, w_{t-1}, w_{t+1}, \cdots, w_{n}$) to predict the masked token $w_t$. \citet{devlin-etal-2019-bert} apply this objective on the concatenated monolingual corpora of 104 languages to get a pre-trained multilingual model (mBERT).\footnote{https://github.com/google-research/bert/blob/master/multilingual.md}

\paragraph{Failings of Masked Language Modeling} While mBERT has shown drastic improvements for several multilingual NLP tasks \cite{hu2020xtreme} \aditi{add more citations}, there are inherent limitations to mBERT's cross-lingual generalization which probably stem from the design of the MLM objective. MLM uses monolingual context to learn contextualized representations which in the multilingual setting can lead to learning inconsistent cross-lingual representations. To verify this hypothesis, we analyze the top-10 MLM predictions from mBERT for four languages, namely Hindi, German, Spanish and English and find that only x\% of those predictions contain synonyms. %\citet{qin2020cosdaml} also 
